CoShNet: A Hybrid Complex Valued Neural Network using Shearlets

In a hybrid neural network, the expensive convolutional layers are replaced by a non-trainable fixed transform with a great reduction in parameters. In previous works, good results were obtained by replacing the convolutions with wavelets. However, wavelet based hybrid network inherited wavelet's lack of vanishing moments along curves and its axis-bias. We propose to use Shearlets with its robust support for important image features like edges, ridges and blobs. The resulting network is called Complex Shearlets Network (CoShNet). It was tested on Fashion-MNIST against ResNet-50 and Resnet-18, obtaining 92.2% versus 90.7% and 91.8% respectively. The proposed network has 49.9k parameters versus ResNet-18 with 11.18m and use 52 times fewer FLOPs. Finally, we trained in under 20 epochs versus 200 epochs required by ResNet and do not need any hyperparameter tuning nor regularization. Code: https://github.com/Ujjawal-K-Panchal/coshnet

==> complex_prob.tex <==

\subsection{Complex Probability logs}
This section deals with logs between \textbf{Complex Probability formula} and \textbf{real\_fc} in \textbf{CoSh-NN} architecture.

\textbf{Note:} All results are calculated for the following configuration:
The dataset in consideration is \href{https://github.com/zalandoresearch/fashion-mnist}{fashion\_mnist}
Outputs from the network are passed through \href{https://pytorch.org/docs/stable/generated/torch.nn.LogSoftmax.html}{$log\_softmax()$} and then passed to \href{https://pytorch.org/docs/stable/nn.functional.html?highlight=functional\%20nll_loss#torch.nn.functional.nll_loss}{$nll\_loss$}; both of which are defined in Pytorch framework.

\subsubsection{real\_fc model}
The \textbf{real\_fc model}, as shown in \cite{Trabelsi2017}, concatenates the real and imaginary part in a tensor and propogates it forward through 1 final $\mathbb{R}$ fully connected layer.

The code for the same is given in image \ref{realfc-code}.


\begin{figure}[htbp]
    \centering
	\includegraphics[width = 70mm]{./images/realfc-arch.png}\\
	\includegraphics[width = 70mm]{./images/realfc-forward.png}
	\caption{above given is code for real-fc implementation. It first concatenates the real and imaginary tensor and propogates it through one final fully connected layer.}
	\label{realfc-code}
\end{figure}

\subsection{cp-nosq model}
The \textbf{cp-nosq} model tries to replicate the architecture given in above realfc model, without an additional layer. \textbf{Also it doesn't square the amplitude, which avoids 0 probabilities for certain events.
}
The code for the same is given below in image \ref{cp-nosq-code}

\begin{figure}[htbp]
    \centering
	\includegraphics[width = 70mm]{./images/cp-nosq-arch.png}\\
	\includegraphics[width = 70mm]{./images/cp-nosq-forward.png}
	\caption{above given is code for cp-nosq implementation. \textbf{Notice how the squaring of magnitude is commented out}.}
	\label{cp-nosq-code}
\end{figure}

\section{cpa-model}\label{cpa-model}
cpa-model stands for complex probability amplitude model. The complex number is interpreted using a function $f: \mathbb{C} \rightarrow \mathbb{R}$ given in eqn. \ref{cpa} as probability density. 

\begin{equation}
	f(z) = |magnitude(z)|^2 \label{cpa}
\end{equation}

Because this formula leads to NaNs in trabelsi-standard initialization due to dying \textsf{relu}, we compare it with other models in a separate model where the activation is changed with the ELU activation function with support for negative response from neurons.
 



